Surface-near domain engineering in multi-domain x-cut lithium niobate tantalate mixed crystals

Lithium niobate and lithium tantalate are among the most widespread materials for nonlinear, integrated photonics. Mixed crystals with arbitrary Nb-Ta ratios provide a new degree of freedom to tune materials properties, such as the birefringence, but also leverage the advantages of the singular compounds, for example, by combining the thermal stability of lithium tantalate with the larger nonlinear or piezoelectric constants of lithium niobate. Periodic poling is the prerequisite for any nonlinear optical application. For mixed crystals this has been challenging so far due to the lack of homogeneous, mono-domain crystals, which severely inhibit domain growth and nucleation. In this work we demonstrate that surface-near ($< 1$~$\mu$m depth) periodic poling on x-cut lithium niobate tantalate mixed crystals can be achieved via electric field poling and lithographically structured electrodes. We find that naturally occurring head-to-head or tail-to-tail domain walls in the as-grown crystal inhibit domain inversion at a larger scale. However, periodic poling is possible, if the gap size between the poling electrodes is of the same order of magnitude or smaller than the average size of naturally occurring domains. This work provides the basis for the nonlinear optical application of lithium niobate tantalate mixed crystals.

==> preamble.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Ab hier ist Platz für eigene Ergänzungen (Pakete, Befehle, etc.)

% Grafiken, Tabellen, Mathematikumgebungen
\usepackage{graphicx,xcolor}
\usepackage{tabularx}
\usepackage{amsmath,amsfonts,amssymb}

%Einheit \SI{}[]{}


% für klickbare Referenzen
\usepackage{acronym}

%Einheit \SI{}[]{}
\usepackage[]{siunitx}

%hyperlinks
\usepackage{hyperref}


%\usepackage[colorlinks=true, 
%urlcolor=green, 
%citecolor=black, 
%linkcolor=black]{hyperref} 
